FacilityAudit-Agent: Beyond Mention-as-Usage for Fine-Grained Facility Contribution Attribution in Astrophysics Publications

Observatory bibliographies increasingly need to determine not only whether a facility is named in a paper, but how its data support the scientific argument. We frame this need as semantic contribution attribution on a six-level scale (L0-L5), from non-use and mention-only cases to auxiliary, major, and exclusive data support. We present FacilityAudit-Agent, a framework that builds a page-bounded outline of each PDF, enriches sections with roles and facility mentions, and uses a tool-calling large language model (LLM) to fetch text on demand. Evidence from the sections is combined through an explicit decision tree and a coverage-calibrated confidence score, with uncertain cases routed to human review. The framework supports both single-facility and inventory audits and transfers to new facilities without retraining. On a test set of 39,358 human-annotated paper-facility pairs, FacilityAudit-Agent achieves 89.1% accuracy and 79.8% macro-F1 in single_audit mode, outperforming the other three baselines by 5.8, 8.3, and 12.1 accuracy points, respectively, with the clearest gains at L2 and L5. In inventory_audit mode, it also leads in facility listing and in level assignment among listed pairs. Ablations show multi-hop reading and tree indexing matter most for L3-L5. FacilityAudit-Agent has been deployed at the National Astronomical Data Center, where it is responsible for processing publications related to LAMOST, FAST, and EP.

==> main_comparison.tex <==
\begin{table*}[t]
\centering
\caption{Main comparison on the test set with DeepSeek-V4-Flash.
Per-level columns are F1 scores (\%).
Best values in each column are in bold.}
\label{tab:main_comparison}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccc}
\hline\hline
Method & L0 & L1 & L2 & L3 & L4 & L5 & Acc & Macro-P & Macro-R & Macro-F1 \\
\hline
Full-context-LLM & 82.0 & 79.5 & 51.3 & 61.0 & 56.5 & 51.9 & 67.0 & 65.7 & 61.8 & 63.7 \\
TRACS-AMC & 73.8 & 73.0 & 43.9 & 60.6 & --- & --- & 49.8 & 42.0 & 43.7 & 41.9 \\
Chunk-RAG & 79.9 & 77.5 & 46.8 & 57.0 & 51.0 & 45.9 & 63.5 & 61.5 & 58.0 & 59.7 \\
FacilityAudit-Agent & \textbf{86.5} & \textbf{85.0} & \textbf{57.4} & \textbf{71.0} & \textbf{69.0} & \textbf{66.5} & \textbf{76.0} & \textbf{74.0} & \textbf{71.2} & \textbf{72.5} \\
\hline
\end{tabular*}
\end{table*}
